Fine-grained Fact Verification with Kernel Graph Attention Network

Fact Verification requires fine-grained natural language inference capability that finds subtle clues to identify the syntactical and semantically correct but not well-supported claims. This paper presents Kernel Graph Attention Network (KGAT), which conducts more fine-grained fact verification with kernel-based attentions. Given a claim and a set of potential evidence sentences that form an evidence graph, KGAT introduces node kernels, which better measure the importance of the evidence node, and edge kernels, which conduct fine-grained evidence propagation in the graph, into Graph Attention Networks for more accurate fact verification. KGAT achieves a 70.38% FEVER score and significantly outperforms existing fact verification models on FEVER, a large-scale benchmark for fact verification. Our analyses illustrate that, compared to dot-product attentions, the kernel-based attention concentrates more on relevant evidence sentences and meaningful clues in the evidence graph, which is the main source of KGAT's effectiveness.

==> appedix.tex <==
\begin{appendix}
\section{Case Study}
Table~\ref{tab:case} shows an example claim whose verification needs to perform reasoning over multiple pieces of evidence. We leverage the same example used by GEAR for fair comparison~\cite{zhou2019gear}. The first two evidence sentences are ground truth evidence.
% which do received higher attention weights from \texttt{Node-Kernel}, as shown by the scores in the end of the sentences.

%We first plot the attention map between different evidence nodes and the selection probability, as shown in Figure~\ref{fig:case:att}. The interaction between evidence nodes is a crucial part for multi-evidence reasoning. Therefore, models need to summarize some information clues from neighbor evidence nodes. On the other hand, the selection probability evaluates which evidence is used to do verification. 

%\texttt{GAT} shows less effective for attention between evidence nodes and evidence node selection attention, as shown in Figure~\ref{fig:case:dgat}. The attention for evidence node interactions usually focus more on evidence selection and separate the main reasoning effort to the evidence selection part. On the contrary, the attention between two evidence nodes of \texttt{KGAT} is more uniform than \texttt{GAT}, as shown in Figure~\ref{fig:case:kgat}, which indicates the kernel fine-grained evidence node representation are all important and useful for the claim label inference. %\cx{I still find it a little weird here. The edge kernels mostly work on selecting the terms (weighting them) in each sentence. Are they really at the node level? It is not as intuitive to analysis them at the node level?}
%The attention between two evidence nodes of \texttt{KGAT} does not stick to select the appropriate evidence for reasoning because our kernel based attention of \texttt{KGAT}-\texttt{Node} can choose the best evidence easily. 

Figure~\ref{fig:case:token} presents the attention distribution on the second evidence, required by the first evidence ($\alpha_i^{2 \rightarrow 1}$). It illustrates how much attention weights evidence (1) puts on evidence (2)'s tokens, in order to gather useful information to update the representation of evidence (1). Darker red colors indicate high attention weights.

% for the second evidence node; the attention weight $\alpha_i^{2 \rightarrow 1}$ is plotted. $\alpha_i^{2 \rightarrow 1}$ represents the second evidence's tokens propagates to the first evidence. The tokens for the second evidence are highlighted with deeper color if they shares more attention. 

The first evidence verifies that ``Al Jardine is an American musician'' but has not enough information to verify ``Al Jardine is a rhythm guitarist''. In \texttt{KGAT}, the edge kernels accurately pick up the information evidence (1) needed from evidence (2): ``rhythm guitarist'', which fills the missing information and completes the reasoning chain. Also, ``Al Jardine'' also receives more attention, which verifies the evidence is about the person in the claim. Such kernel attention is more intuitive and effective than the dot-product attention in GAT, where the attention is scattered almost uniformly across all tokens, similar to the observations in recent research~\cite{clark2019does}.
% more weight than other tokens. Both these two phrases are also necessary clues which indicate the person name and the modifier for \textit{Al Jardine}'s occupation.
% For the evidence \textt{Edge}, kernels present attention patterns which better which focus on the important tokens, which is dropped by the first evidence. 

% This focused attention is more effective and intuitive than the scattered attention from dot product attention.

% Benefiting from \texttt{KGAT}-\texttt{Edge} and \texttt{KGAT}-\texttt{Node}, these two individual but collaborative modules, \texttt{KGAT} performs a fine-grained reasoning by summarizing some important clues from other nodes.
%and powerful selection, which leads to a better performance, especially for the multiple evidence reasoning scenario.

\input{table/case.tex}
%\input{figure/case.tex}
\input{figure/case_token.tex}
\end{appendix}

==> figure/case.tex <==
\begin{figure}[t]
    \centering
    \subfigure[DGAT model.] { \label{fig:case:dgat} 
    \includegraphics[width=0.45\linewidth]{image/case_gat.png}}
    \subfigure[KGAT model.] { \label{fig:case:kgat} 
    \includegraphics[width=0.45\linewidth]{image/case_kgat.png}}
    \caption{Attention map for the case in Table~\ref{tab:case}. The first five rows indicate the attention weights from evidence nodes from 1 to 5 (Edge Weight) and the last row shows the selection weights (Node Weight).}
    \label{fig:case:att}
\end{figure}
